A Tactile Sensing Foot for Single Robot Leg Stabilization

Tactile sensing on human feet is crucial for motion control, however, has not been explored in robotic counterparts. This work is dedicated to endowing tactile sensing to legged robot's feet and showing that a single-legged robot can be stabilized with only tactile sensing signals from its foot. We propose a robot leg with a novel vision-based tactile sensing foot system and implement a processing algorithm to extract contact information for feedback control in stabilizing tasks. A pipeline to convert images of the foot skin into high-level contact information using a deep learning framework is presented. The leg was quantitatively evaluated in a stabilization task on a tilting surface to show that the tactile foot was able to estimate both the surface tilting angle and the foot poses. Feasibility and effectiveness of the tactile system were investigated qualitatively in comparison with conventional single-legged robotic systems using inertia measurement units (IMU). Experiments demonstrate the capability of vision-based tactile sensors in assisting legged robots to maintain stability on unknown terrains and the potential for regulating more complex motions for humanoid robots.

==> sections/Grasping_tasks.tex <==
% !TeX spellcheck = en_GB

\section{Grasping Tasks}

\begin{figure}
	\centering
	\includegraphics[width=0.485\textwidth]{friction_data.png}
	\caption{Contact force signals under multiple sliding motion trials. Upper right chart is generated by measuring ratios $F_t/F_n$ at peaks of $F_t$ (as blue circles marked). Lower right chart is the ratio $F_t/F_n$ inside the window delineated in purple dash rectangle.}
	\label{friction_data}
	\vspace{-0.3cm}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.35\textwidth]{grasping_setup.png}
	\caption{Adaptive grasping force control experiment. (a). Robotiq 2-finger 140 gripper with FingerVision as fingertips holding an object and then the object is pressed by hand till slip occurs. (b). Gripper with FingerVision holds an object and then the tangential load is increased/decreased by loading and unloading weights on top of the object. }
	\label{grasping_setup}
	\vspace{-0.3cm}
\end{figure}

In this section, effectiveness of the proposed contact force and torque estimation method for vision-based sensors is tested in grasping tasks. Sensing and visualization of contact information as well as adaptive control under external disturbances have been challenging tasks in robotic manipulation. Besides, situations are even more complex when introducing soft contact that brings in nonlinearity in deformation. Fig. \ref{friction_data} shows tangential force and normal force signals during multiple surface sliding trials (data collected by ATI nano-17 Force/Torque sensor). It is noticed from the chart on the upper right in Fig. \ref{friction_data} that the friction coefficient (equals to the ratio of tangential and normal forces $F_t/F_n$ when tangential force reaches each peak, as marked by blue circles) does not remain constant under different normal forces, which is one of the significant properties differences between hyperelastic contact and rigid contact. It also shows that within each trial of surface sliding, the ratio $F_t/F_n$ follows similar evolution: the ratio first rises; once reaches the maximum static friction coefficient, the ratio vibrates in a narrow band; the ratio drops afterwards, suggesting the occurrence of shear slip, as exhibited in the lower right chart of Fig. \ref{friction_data}. 



\subsection{Grasping Stability Visualization}






Taking behavior of $F_t/F_n$ during slip phases into consideration, we implement a visualization system for monitoring of grasping force and slip, as shown in Fig. \ref{contact_phase_transitions}. Since the friction coefficient is not constant, we take the average of friction coefficients across working range of normal force as the nominal value for simplification and visually illustrate friction cones \cite{mason2001mechanics} with this coefficient. The FingerVision sensors are installed on Robotiq 2-finger 140 gripper, serving as finger tips and sensing units, mimicking human fingertips. With the force and torque estimation module, we illustrate transitions of contact phases by classifying the spaces where contact force vectors reside w.r.t. the friction cones. As given in Fig. \ref{contact_phase_transitions}(a), contact statuses are classified into 4 phases: 1) Stable contact; 2) Incipient slip; 3) Slipping; 4) Recovery phase when force vector is regulated back into the yellow or green regions. In Fig. \ref{contact_phase_transitions}(b) contact forces are shown as arrows in green (when the vectors are within the friction cones) and red (outside of the  friction cones). The capability of indicating contact phases is beneficial to grasp reconfiguration for stable grasp.


 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\subsection{Feedback Control of Grasping Force}





In-hand manipulations of objects usually require minimal grasping forces, because the contact condition keeps switching between unstable and stable statuses, e.g. pen rolling in human hand. And when picking up fragile objects, power grasps also need to be avoided. Thus, adaptive control for grasping force is critical in many scenarios. Here we implement a simple feedback controller that takes in contact force estimation and maintains the ratios $F_t/F_n$ in a band on the peripheries of the friction cones (visualized with nominal friction coefficients as described previously). Details of the controller are given in Algorithm \ref{ag:controller}. In the algorithm, variables with subscripts \textit{l} and \textit{r} belong to the left and right contacts.  A conservative control strategy is implemented in our work. To maintain the contact forces in the vicinity of friction cone margins, the gripper decreases the opening if both left and right forces exceed the upper limits of band of the cones and increases the opening while both left and right forces are lower than the lower limits. 

\begin{algorithm}
	\caption{Grasping force controller}
	\hspace*{\algorithmicindent} \textbf{Input:} Contact forces  $F_l$, $F_r$; Gripper opening $D_g$;  \\
	\hspace*{\algorithmicindent} \quad \quad  \quad Band width $d$; Friction coefficient $\mu$.\\
	\hspace*{\algorithmicindent} \textbf{Output:} Gripper requested opening $D_r$.
	\label{pseudoPSO}
	\begin{algorithmic}[1]
		\State Initialize $r_l$, $r_r$ with $\mu$
		\While {True}
		\State $r_l \gets F_{lt}/F_{ln}$, $r_r \gets F_{rt}/F_{rn}$
		
		\If{$r_l > \mu+d/2$ \textbf{and} $r_r > \mu+d/2$ }
		\State $D_r = D_g - 1$
		\EndIf
		
		\If{$r_l < \mu+d/2$ \textbf{and} $r_r < \mu+d/2$ }
		\State $D_r = D_g + 1$
		\EndIf
		
		\EndWhile
	\end{algorithmic}
	\label{ag:controller}
\end{algorithm}


\begin{figure}
	\centering
	\includegraphics[width=0.475\textwidth]{contact_phases.png}
	\caption{Schematic diagram of contact phases and visualization for experiment in Fig. \ref{grasping_setup}(a). Force signals are plotted in Fig. \ref{grasping_plots}(a-b).}
	\label{contact_phase_transitions}
	\vspace{-0.3cm}
\end{figure}


The controller performs well in maintaining stable contact using minimal grasping forces in the object holding experiment during loading and unloading of weights that result in increase and decrease of tangential forces. As demonstrated in Fig. \ref{grasping_plots}(c-d), with controller being active, there are no or much shorter periods of crossovers(indicated as periods when $F_t/F_n$ dramatically rises that leads to contact slip). The ratio $F_t/F_n$ in right-side fingertip recovers quickly from the crossover region (rendered in yellow in Fig. \ref{grasping_plots}) due to the regulation of the force controller. The regulation process can also be seen from the visualization system, which keeps the contact force vectors around the margins of friction cones. Without force control, there is an extended longer period of crossover during loading process. The gripper fails to maintain contact forces inside the friction cones. Grasp fails if at least one contact breaks. It is worth noting that after slip happens on the surface, another crossover occurs due to the fact that dynamic friction coefficient is lower than static friction coefficient. The signals of left and right sensors are not of exactly the same forms, which could stem from the variances in sensor fabrication and calibration, object alignment difference for two contact surfaces and gripper pose not being exactly upright that leads to imbalanced loads on two fingertips.



\begin{figure}
	\centering
	\includegraphics[width=0.485\textwidth]{implement_plots.png}
	\caption{Grasping contact force signals under loads. Force x, y and z are the projections of the contact force onto the sensor surface coordinate system in Fig. \ref{calibration_setup}. (a-b). Changes of contact forces for manual press on grasped object, with constant opening distance between two fingertips. Four contact phases are illustrated in different colors. (c-d). Contact force signals during loading and unloading, with active grasp force controller. (e-f). Contact force signals during loading, without  grasping force controller. The unloading process is not given since contacts are broken, which leads to grasping failure.}
	\label{grasping_plots}
	\vspace{-0.4cm}
\end{figure}











